EEGDash Corpus: A Training-Ready Public Corpus for EEG Foundation Models

Electroencephalography (EEG) foundation models are pretrained on tens of thousands of hours. The largest clinical archives restrict redistribution, while public datasets use different formats and licences. Here, we rebuild the 77 redistributable datasets of the REVE pretraining corpus that reach its 200 Hz input (14,075 hours across 7,272 subjects) and release them as eegdash-corpus-v0, with raw-file access by name through EEGDash and a checksummed Zarr store on Hugging Face, converted with REVE's preprocessing recipe. Every dataset keeps its licence, and any subset of datasets can be selected by name. To test whether this public store pretrains REVE-Base, we train the model twice from scratch with REVE's trainer and score it on seven public OpenEEGBench tasks. First, under linear probing, the frozen encoder reaches 0.331 in chance-adjusted balanced accuracy, against 0.333 for the released model (untrained: 0.200), a difference smaller than the spread between our two pretraining seeds. Second, after fine-tuning, it reaches 0.273 against 0.325 published (0.301 in our rerun), and part of this gap comes from the scoring pipeline. A public, training-ready EEG corpus can therefore pretrain the frozen representations of a foundation model and provide a shared base that other groups can audit.

==> figures/pipeline_traces.tex <==
% Generated by lanes/r3-diagram/scratch/make_traces.py; see the header of pipeline.tex for the sources.
\def\reveRawA{(0,-91) (5,3) (5,1) (10,-90) (10,-90) (15,1) (15,-6) (20,-95) (20,-84) (25,3) (25,-1) (30,-91) (30,-88) (35,1) (35,7) (40,-80) (40,-85) (45,9) (45,10) (50,-83) (50,-85) (55,6) (55,7) (60,-91) (60,-77) (65,12) (65,8) (70,-86) (70,-75) (75,36) (75,54) (80,-50) (80,-26) (85,60) (85,57) (90,-48) (90,-65) (95,32) (95,19) (100,-79) (100,-90) (105,5) (105,-4) (110,-98) (110,-95) (115,-3) (115,-4) (120,-104) (120,-93) (125,-4) (125,-6) (130,-94) (130,-92) (135,-2) (135,-6) (140,-97) (140,-96) (145,-2) (145,-1) (150,-89) (150,-94) (155,-2) (155,-4) (160,-98) (160,-98) (165,-5) (165,-2) (170,-94) (170,-93) (175,-2) (175,-3) (180,-102) (180,-101) (185,-8) (185,-10) (190,-99) (190,-96) (195,-7) (195,-10) (200,-104) (200,-87) (205,3) (205,3) (210,-90) (210,-92) (215,3) (215,-1) (220,-94) (220,-93) (225,1) (225,2) (230,-93) (230,-95) (235,9) (235,1) (240,-91) (240,-87) (245,6) (245,-1) (250,-93) (250,-84) (255,5) (255,0) (260,-88) (260,-92) (265,-3) (265,0) (270,-91) (270,-89) (275,-1) (275,6) (280,-85) (280,-85) (285,6) (285,2) (290,-83) (290,-81) (295,12) (295,4) (300,-89) (300,-87) (305,8) (305,-2) (310,-92) (310,-95) (315,-5) (315,-4) (320,-98) (320,-98) (325,-5) (325,1) (330,-97) (330,-91) (335,0) (335,1) (340,-91) (340,-85) (345,5) (345,24) (350,-83) (350,-50) (355,40) (355,51) (360,-43) (360,-29) (365,66) (365,65) (370,-25) (370,-25) (375,69) (375,77) (380,-25) (380,-8) (385,82) (385,89) (390,-7) (390,-11) (395,81) (395,70) (400,-23) (400,-19) (405,70) (405,61) (410,-28) (410,-21) (415,70) (415,64) (420,-26) (420,-19) (425,70) (425,66) (430,-24) (430,-16) (435,71) (435,69) (440,-19) (440,-26) (445,67) (445,69) (450,-29) (450,-22) (455,68) (455,75) (460,-17) (460,-17) (465,74) (465,71) (470,-19) (470,-21) (475,76) (475,80) (480,-14) (480,-21) (485,75) (485,77) (490,-22) (490,-20) (495,73) (495,76) (500,-25) (500,-24) (505,66) (505,64) (510,-30) (510,-24) (515,69) (515,69) (520,-25) (520,-14) (525,75) (525,81) (530,-13) (530,-10) (535,81) (535,79) (540,-11) (540,-8) (545,82) (545,81) (550,-12) (550,-6) (555,86) (555,76) (560,-15) (560,-8) (565,81) (565,74) (570,-16) (570,-18) (575,76) (575,74) (580,-18) (580,-13) (585,76) (585,78) (590,-15) (590,-7) (595,85) (595,83) (600,-9) (600,-11) (605,86) (605,87) (610,-13) (610,-12) (615,88) (615,85) (620,-9) (620,-12) (625,81) (625,76) (630,-18) (630,-16) (635,75) (635,83) (640,-12) (640,-13) (645,80) (645,80) (650,-16) (650,-14) (655,77) (655,76) (660,-17) (660,-17) (665,74) (665,82) (670,-12) (670,-12) (675,86) (675,85) (680,-8) (680,-8) (685,84) (685,88) (690,-4) (690,-3) (695,88) (695,81) (700,-7) (700,-8) (705,84) (705,83) (710,-11) (710,-16) (715,80) (715,80) (720,-17) (720,-11) (725,77) (725,78) (730,-14) (730,-14) (735,72) (735,79) (740,-10) (740,-15) (745,72) (745,75) (750,-18) (750,-17) (755,71) (755,79) (760,-15) (760,-19) (765,78) (765,76) (770,-17) (770,-17) (775,75) (775,84) (780,-14) (780,-18) (785,74) (785,78) (790,-15) (790,-15) (795,80) (795,76) (800,-19) (800,-18) (805,81) (805,87) (810,-6) (810,-6) (815,82) (815,84) (820,-17) (820,-14) (825,82) (825,79) (830,-17) (830,-26) (835,71) (835,76) (840,-15) (840,-21) (845,69) (845,79) (850,-15) (850,-12) (855,79) (855,75) (860,-26) (860,-20) (865,70) (865,63) (870,-21) (870,-23) (875,70) (875,72) (880,-18) (880,-14) (885,77) (885,77) (890,-10) (890,-17) (895,76) (895,67) (900,-21) (900,-15) (905,81) (905,75) (910,-17) (910,-22) (915,81) (915,76) (920,-20) (920,-17) (925,75) (925,70) (930,-19) (930,-29) (935,64) (935,58) (940,-36) (940,-38) (945,60) (945,53) (950,-37) (950,-36) (955,60) (955,50) (960,-45) (960,-42) (965,54) (965,55) (970,-40) (970,-49) (975,47) (975,54) (980,-39) (980,-38) (985,66) (985,72) (990,-22) (990,-18) (995,75) (995,85) (1000,-9)}
\def\reveRawB{(0,-160) (5,-91) (5,-80) (10,-143) (10,-142) (15,-78) (15,-95) (20,-153) (20,-129) (25,-75) (25,-83) (30,-141) (30,-134) (35,-76) (35,-62) (40,-121) (40,-126) (45,-60) (45,-63) (50,-125) (50,-128) (55,-68) (55,-71) (60,-136) (60,-113) (65,-53) (65,-65) (70,-127) (70,-117) (75,-26) (75,18) (80,-76) (80,-30) (85,18) (85,10) (90,-73) (90,-106) (95,-41) (95,-55) (100,-133) (100,-149) (105,-73) (105,-96) (110,-160) (110,-160) (115,-101) (115,-108) (120,-160) (120,-160) (125,-106) (125,-105) (130,-160) (130,-160) (135,-96) (135,-107) (140,-160) (140,-160) (145,-105) (145,-91) (150,-158) (150,-160) (155,-107) (155,-114) (160,-160) (160,-160) (165,-121) (165,-106) (170,-160) (170,-160) (175,-111) (175,-126) (180,-160) (180,-160) (185,-130) (185,-138) (190,-160) (190,-160) (195,-131) (195,-136) (200,-160) (200,-160) (205,-101) (205,-94) (210,-160) (210,-160) (215,-96) (215,-107) (220,-160) (220,-160) (225,-110) (225,-104) (230,-160) (230,-160) (235,-83) (235,-100) (240,-160) (240,-149) (245,-84) (245,-96) (250,-159) (250,-158) (255,-84) (255,-95) (260,-156) (260,-158) (265,-99) (265,-95) (270,-158) (270,-160) (275,-92) (275,-85) (280,-151) (280,-156) (285,-81) (285,-86) (290,-146) (290,-149) (295,-67) (295,-92) (300,-160) (300,-160) (305,-90) (305,-115) (310,-160) (310,-160) (315,-118) (315,-118) (320,-160) (320,-160) (325,-117) (325,-108) (330,-160) (330,-160) (335,-107) (335,-105) (340,-160) (340,-160) (345,-107) (345,-71) (350,-160) (350,-101) (355,-34) (355,2) (360,-70) (360,-42) (365,27) (365,33) (370,-30) (370,-19) (375,47) (375,69) (380,-24) (380,15) (385,74) (385,91) (390,21) (390,6) (395,79) (395,44) (400,-21) (400,-16) (405,47) (405,28) (410,-34) (410,-13) (415,51) (415,45) (420,-20) (420,-14) (425,61) (425,49) (430,-16) (430,-7) (435,55) (435,55) (440,-9) (440,-24) (445,49) (445,54) (450,-28) (450,-21) (455,46) (455,62) (460,-4) (460,1) (465,61) (465,60) (470,0) (470,-14) (475,49) (475,55) (480,-5) (480,-19) (485,55) (485,60) (490,-21) (490,-16) (495,41) (495,50) (500,-35) (500,-32) (505,28) (505,29) (510,-36) (510,-27) (515,43) (515,36) (520,-31) (520,-15) (525,45) (525,54) (530,-16) (530,-12) (535,54) (535,64) (540,-2) (540,-2) (545,63) (545,68) (550,-6) (550,15) (555,81) (555,61) (560,1) (560,6) (565,73) (565,38) (570,-24) (570,-26) (575,41) (575,33) (580,-29) (580,-18) (585,45) (585,45) (590,-26) (590,-2) (595,63) (595,64) (600,-12) (600,-8) (605,73) (605,73) (610,-5) (610,-3) (615,72) (615,71) (620,-4) (620,-2) (625,66) (625,56) (630,-11) (630,-5) (635,51) (635,62) (640,-4) (640,4) (645,65) (645,60) (650,-10) (650,-7) (655,66) (655,52) (660,-12) (660,-13) (665,49) (665,60) (670,-6) (670,1) (675,68) (675,68) (680,4) (680,12) (685,75) (685,71) (690,9) (690,17) (695,73) (695,69) (700,12) (700,1) (705,66) (705,64) (710,-12) (710,-7) (715,68) (715,78) (720,-6) (720,8) (725,72) (725,65) (730,0) (730,-4) (735,63) (735,83) (740,21) (740,7) (745,68) (745,66) (750,12) (750,7) (755,65) (755,84) (760,11) (760,9) (765,86) (765,80) (770,13) (770,9) (775,69) (775,92) (780,15) (780,4) (785,80) (785,80) (790,15) (790,19) (795,93) (795,73) (800,2) (800,12) (805,77) (805,91) (810,20) (810,25) (815,86) (815,84) (820,3) (820,9) (825,80) (825,73) (830,2) (830,-18) (835,59) (835,65) (840,-5) (840,-1) (845,56) (845,66) (850,8) (850,1) (855,69) (855,57) (860,-21) (860,-14) (865,59) (865,38) (870,-18) (870,-21) (875,40) (875,43) (880,-21) (880,-14) (885,53) (885,53) (890,-5) (890,-22) (895,49) (895,34) (900,-30) (900,-13) (905,59) (905,50) (910,-18) (910,-30) (915,66) (915,47) (920,-29) (920,-13) (925,54) (925,35) (930,-17) (930,-43) (935,16) (935,9) (940,-50) (940,-70) (945,2) (945,-4) (950,-62) (950,-63) (955,13) (955,5) (960,-76) (960,-64) (965,-1) (965,8) (970,-62) (970,-82) (975,-14) (975,1) (980,-63) (980,-52) (985,28) (985,29) (990,-32) (990,-41) (995,38) (995,57) (1000,-11)}
\def\reveRawC{(0,-59) (5,35) (5,32) (10,-59) (10,-62) (15,31) (15,26) (20,-66) (20,-57) (25,38) (25,25) (30,-71) (30,-59) (35,33) (35,35) (40,-57) (40,-57) (45,40) (45,43) (50,-58) (50,-59) (55,39) (55,29) (60,-68) (60,-51) (65,45) (65,37) (70,-58) (70,-51) (75,52) (75,63) (80,-33) (80,-24) (85,66) (85,70) (90,-41) (90,-49) (95,45) (95,45) (100,-59) (100,-71) (105,32) (105,18) (110,-81) (110,-75) (115,20) (115,22) (120,-76) (120,-71) (125,24) (125,22) (130,-67) (130,-69) (135,25) (135,26) (140,-70) (140,-74) (145,36) (145,34) (150,-60) (150,-63) (155,31) (155,28) (160,-67) (160,-69) (165,26) (165,31) (170,-64) (170,-60) (175,33) (175,37) (180,-66) (180,-68) (185,30) (185,21) (190,-70) (190,-59) (195,33) (195,26) (200,-70) (200,-61) (205,35) (205,38) (210,-60) (210,-67) (215,37) (215,36) (220,-61) (220,-77) (225,33) (225,28) (230,-67) (230,-67) (235,48) (235,34) (240,-63) (240,-53) (245,41) (245,26) (250,-67) (250,-56) (255,38) (255,27) (260,-63) (260,-67) (265,24) (265,25) (270,-71) (270,-62) (275,32) (275,39) (280,-51) (280,-56) (285,42) (285,36) (290,-56) (290,-41) (295,54) (295,41) (300,-60) (300,-58) (305,47) (305,39) (310,-66) (310,-62) (315,33) (315,30) (320,-70) (320,-70) (325,27) (325,35) (330,-62) (330,-57) (335,40) (335,31) (340,-61) (340,-52) (345,36) (345,48) (350,-57) (350,-46) (355,45) (355,62) (360,-41) (360,-35) (365,67) (365,69) (370,-27) (370,-16) (375,83) (375,89) (380,-14) (380,-1) (385,95) (385,91) (390,-6) (390,-15) (395,78) (395,76) (400,-21) (400,-22) (405,74) (405,61) (410,-32) (410,-28) (415,68) (415,63) (420,-32) (420,-18) (425,78) (425,73) (430,-26) (430,-16) (435,79) (435,79) (440,-22) (440,-26) (445,72) (445,77) (450,-27) (450,-30) (455,67) (455,76) (460,-19) (460,-18) (465,75) (465,77) (470,-16) (470,-18) (475,79) (475,89) (480,-13) (480,-30) (485,70) (485,82) (490,-19) (490,-23) (495,71) (495,83) (500,-23) (500,-29) (505,61) (505,54) (510,-40) (510,-33) (515,63) (515,67) (520,-34) (520,-24) (525,71) (525,82) (530,-20) (530,-21) (535,81) (535,74) (540,-23) (540,-13) (545,79) (545,78) (550,-20) (550,-20) (555,79) (555,65) (560,-30) (560,-26) (565,73) (565,67) (570,-34) (570,-36) (575,70) (575,64) (580,-37) (580,-25) (585,65) (585,66) (590,-31) (590,-20) (595,77) (595,72) (600,-20) (600,-27) (605,80) (605,70) (610,-31) (610,-34) (615,71) (615,69) (620,-30) (620,-33) (625,64) (625,63) (630,-43) (630,-37) (635,56) (635,66) (640,-35) (640,-38) (645,61) (645,67) (650,-39) (650,-38) (655,55) (655,57) (660,-39) (660,-39) (665,54) (665,64) (670,-36) (670,-41) (675,54) (675,56) (680,-42) (680,-41) (685,55) (685,71) (690,-23) (690,-29) (695,69) (695,54) (700,-35) (700,-36) (705,61) (705,56) (710,-43) (710,-48) (715,59) (715,54) (720,-50) (720,-48) (725,54) (725,54) (730,-48) (730,-39) (735,50) (735,56) (740,-40) (740,-47) (745,45) (745,45) (750,-51) (750,-53) (755,39) (755,42) (760,-57) (760,-54) (765,44) (765,53) (770,-50) (770,-51) (775,46) (775,50) (780,-50) (780,-54) (785,36) (785,54) (790,-42) (790,-49) (795,47) (795,54) (800,-46) (800,-46) (805,56) (805,67) (810,-29) (810,-43) (815,52) (815,55) (820,-50) (820,-47) (825,51) (825,55) (830,-49) (830,-67) (835,40) (835,47) (840,-50) (840,-59) (845,33) (845,59) (850,-44) (850,-44) (855,49) (855,49) (860,-64) (860,-56) (865,45) (865,37) (870,-53) (870,-64) (875,44) (875,46) (880,-54) (880,-51) (885,45) (885,38) (890,-51) (890,-61) (895,40) (895,23) (900,-66) (900,-63) (905,39) (905,30) (910,-67) (910,-78) (915,37) (915,33) (920,-70) (920,-74) (925,22) (925,21) (930,-73) (930,-83) (935,13) (935,11) (940,-95) (940,-90) (945,6) (945,4) (950,-92) (950,-89) (955,18) (955,10) (960,-88) (960,-88) (965,19) (965,23) (970,-84) (970,-92) (975,10) (975,22) (980,-76) (980,-78) (985,25) (985,42) (990,-60) (990,-58) (995,37) (995,45) (1000,-53)}
\def\reveRawD{(0,-160) (5,-112) (5,-72) (10,-149) (10,-155) (15,-73) (15,-89) (20,-160) (20,-147) (25,-62) (25,-78) (30,-131) (30,-110) (35,-55) (35,-50) (40,-116) (40,-117) (45,-47) (45,-29) (50,-128) (50,-101) (55,-48) (55,-40) (60,-110) (60,-100) (65,-34) (65,-58) (70,-108) (70,-116) (75,-55) (75,-26) (80,-130) (80,-95) (85,-41) (85,-46) (90,-89) (90,-142) (95,-61) (95,-43) (100,-132) (100,-137) (105,-65) (105,-63) (110,-160) (110,-143) (115,-85) (115,-89) (120,-160) (120,-139) (125,-67) (125,-82) (130,-154) (130,-135) (135,-69) (135,-84) (140,-136) (140,-154) (145,-90) (145,-82) (150,-134) (150,-138) (155,-89) (155,-104) (160,-150) (160,-160) (165,-109) (165,-96) (170,-146) (170,-157) (175,-113) (175,-121) (180,-160) (180,-160) (185,-116) (185,-109) (190,-160) (190,-159) (195,-111) (195,-111) (200,-160) (200,-134) (205,-76) (205,-44) (210,-143) (210,-132) (215,-65) (215,-75) (220,-145) (220,-146) (225,-45) (225,-38) (230,-147) (230,-100) (235,-12) (235,-57) (240,-117) (240,-131) (245,-25) (245,-57) (250,-132) (250,-145) (255,-57) (255,-30) (260,-119) (260,-125) (265,-57) (265,-45) (270,-124) (270,-128) (275,-61) (275,-58) (280,-132) (280,-90) (285,-5) (285,-1) (290,-92) (290,-101) (295,17) (295,-20) (300,-111) (300,-139) (305,-26) (305,-62) (310,-113) (310,-137) (315,-38) (315,-37) (320,-156) (320,-133) (325,-45) (325,-73) (330,-160) (330,-119) (335,-38) (335,-53) (340,-127) (340,-119) (345,-48) (345,-19) (350,-123) (350,-73) (355,-10) (355,12) (360,-50) (360,-45) (365,23) (365,8) (370,-48) (370,-54) (375,24) (375,63) (380,-62) (380,8) (385,63) (385,85) (390,27) (390,4) (395,94) (395,55) (400,-31) (400,-21) (405,70) (405,39) (410,-49) (410,-9) (415,58) (415,102) (420,-21) (420,-12) (425,103) (425,104) (430,-17) (430,-11) (435,111) (435,99) (440,-7) (440,-19) (445,77) (445,109) (450,16) (450,-5) (455,104) (455,128) (460,-19) (460,44) (465,111) (465,42) (470,-27) (470,-12) (475,53) (475,52) (480,-15) (480,-5) (485,68) (485,78) (490,-13) (490,-22) (495,70) (495,62) (500,-35) (500,-21) (505,90) (505,65) (510,-2) (510,-16) (515,98) (515,96) (520,-22) (520,-2) (525,68) (525,79) (530,10) (530,-29) (535,104) (535,108) (540,-14) (540,26) (545,85) (545,77) (550,-12) (550,40) (555,105) (555,85) (560,17) (560,13) (565,96) (565,30) (570,-32) (570,-28) (575,41) (575,31) (580,-30) (580,-26) (585,61) (585,37) (590,-33) (590,8) (595,98) (595,85) (600,-51) (600,-4) (605,104) (605,105) (610,-6) (610,44) (615,106) (615,92) (620,37) (620,27) (625,96) (625,92) (630,-8) (630,-13) (635,101) (635,96) (640,-30) (640,-27) (645,102) (645,96) (650,-48) (650,-2) (655,98) (655,46) (660,-10) (660,6) (665,58) (665,62) (670,-7) (670,22) (675,92) (675,77) (680,0) (680,0) (685,96) (685,54) (690,-1) (690,21) (695,71) (695,80) (700,14) (700,-9) (705,67) (705,62) (710,-14) (710,-10) (715,99) (715,78) (720,17) (720,13) (725,75) (725,85) (730,6) (730,-5) (735,54) (735,103) (740,19) (740,-31) (745,79) (745,104) (750,30) (750,6) (755,91) (755,107) (760,38) (760,41) (765,137) (765,111) (770,37) (770,18) (775,104) (775,137) (780,39) (780,43) (785,129) (785,127) (790,60) (790,37) (795,131) (795,60) (800,-17) (800,39) (805,103) (805,120) (810,-12) (810,26) (815,139) (815,113) (820,15) (820,10) (825,110) (825,126) (830,50) (830,16) (835,72) (835,94) (840,15) (840,21) (845,106) (845,86) (850,-2) (850,5) (855,121) (855,48) (860,-6) (860,-11) (865,56) (865,48) (870,6) (870,-26) (875,38) (875,45) (880,-19) (880,-21) (885,45) (885,72) (890,-2) (890,-17) (895,65) (895,43) (900,-17) (900,6) (905,70) (905,53) (910,-9) (910,-44) (915,106) (915,32) (920,-54) (920,-58) (925,68) (925,37) (930,-49) (930,-49) (935,30) (935,18) (940,-34) (940,-93) (945,-40) (945,10) (950,-69) (950,-94) (955,6) (955,46) (960,-101) (960,-81) (965,1) (965,2) (970,-74) (970,-71) (975,-7) (975,-1) (980,-94) (980,-50) (985,17) (985,-5) (990,-59) (990,-90) (995,-15) (995,19) (1000,-61)}
\def\reveRawE{(0,-144) (5,-82) (5,-71) (10,-141) (10,-118) (15,-27) (15,-73) (20,-160) (20,-160) (25,-72) (25,-75) (30,-130) (30,-140) (35,-70) (35,-76) (40,-139) (40,-138) (45,-92) (45,-82) (50,-146) (50,-146) (55,-93) (55,-88) (60,-142) (60,-138) (65,-85) (65,-103) (70,-151) (70,-160) (75,-116) (75,-137) (80,-160) (80,-160) (85,-148) (85,-138) (90,-160) (90,-160) (95,-122) (95,-125) (100,-160) (100,-149) (105,-79) (105,-47) (110,-106) (110,-124) (115,-70) (115,-61) (120,-135) (120,-117) (125,-51) (125,-60) (130,-137) (130,-107) (135,-50) (135,-62) (140,-124) (140,-116) (145,-46) (145,-87) (150,-126) (150,-135) (155,-73) (155,-70) (160,-123) (160,-135) (165,-67) (165,-71) (170,-120) (170,-135) (175,-80) (175,-97) (180,-157) (180,-137) (185,-77) (185,-70) (190,-148) (190,-153) (195,-95) (195,-70) (200,-138) (200,-114) (205,-46) (205,-61) (210,-122) (210,-97) (215,-34) (215,-52) (220,-146) (220,-121) (225,-31) (225,-27) (230,-84) (230,-62) (235,-20) (235,-56) (240,-116) (240,-87) (245,-36) (245,-16) (250,-105) (250,-133) (255,-83) (255,-63) (260,-126) (260,-130) (265,-66) (265,-58) (270,-117) (270,-128) (275,-60) (275,-57) (280,-116) (280,-98) (285,-12) (285,14) (290,-67) (290,-53) (295,20) (295,4) (300,-51) (300,-71) (305,-7) (305,12) (310,-38) (310,-66) (315,30) (315,29) (320,-29) (320,-34) (325,30) (325,-12) (330,-90) (330,-30) (335,26) (335,34) (340,-23) (340,-26) (345,39) (345,53) (350,-17) (350,-2) (355,51) (355,60) (360,-5) (360,-27) (365,41) (365,1) (370,-49) (370,-87) (375,-11) (375,-11) (380,-90) (380,-62) (385,1) (385,10) (390,-53) (390,-53) (395,36) (395,3) (400,-67) (400,-19) (405,54) (405,63) (410,-61) (410,-29) (415,73) (415,93) (420,-27) (420,-19) (425,97) (425,76) (430,-12) (430,0) (435,86) (435,117) (440,45) (440,29) (445,115) (445,116) (450,34) (450,69) (455,149) (455,90) (460,11) (460,18) (465,102) (465,29) (470,-54) (470,-2) (475,39) (475,24) (480,-28) (480,-1) (485,93) (485,51) (490,-19) (490,-16) (495,82) (495,73) (500,-7) (500,-2) (505,123) (505,77) (510,31) (510,22) (515,80) (515,81) (520,16) (520,-2) (525,63) (525,47) (530,-27) (530,-60) (535,57) (535,50) (540,-74) (540,-30) (545,65) (545,31) (550,-61) (550,13) (555,86) (555,50) (560,-9) (560,-1) (565,71) (565,57) (570,-9) (570,-13) (575,40) (575,23) (580,-48) (580,-45) (585,7) (585,19) (590,-60) (590,-47) (595,30) (595,28) (600,-52) (600,-31) (605,28) (605,35) (610,-49) (610,-14) (615,45) (615,26) (620,-44) (620,-33) (625,45) (625,65) (630,-54) (630,-55) (635,69) (635,45) (640,-67) (640,-63) (645,64) (645,52) (650,-104) (650,-48) (655,64) (655,39) (660,-79) (660,-58) (665,50) (665,-2) (670,-76) (670,-48) (675,24) (675,-6) (680,-68) (680,-59) (685,25) (685,-10) (690,-73) (690,-44) (695,42) (695,48) (700,-3) (700,-22) (705,61) (705,83) (710,-8) (710,-40) (715,65) (715,101) (720,0) (720,-42) (725,45) (725,84) (730,10) (730,-52) (735,32) (735,51) (740,-43) (740,-95) (745,46) (745,105) (750,-6) (750,-34) (755,80) (755,85) (760,11) (760,24) (765,93) (765,78) (770,-3) (770,14) (775,78) (775,91) (780,32) (780,10) (785,92) (785,72) (790,-3) (790,23) (795,81) (795,58) (800,-17) (800,22) (805,92) (805,70) (810,-16) (810,43) (815,116) (815,70) (820,15) (820,35) (825,101) (825,95) (830,48) (830,42) (835,117) (835,100) (840,44) (840,36) (845,108) (845,87) (850,12) (850,8) (855,92) (855,62) (860,-9) (860,-20) (865,44) (865,41) (870,10) (870,-14) (875,52) (875,64) (880,8) (880,-37) (885,48) (885,89) (890,-21) (890,-12) (895,86) (895,83) (900,27) (900,23) (905,86) (905,90) (910,9) (910,9) (915,94) (915,46) (920,4) (920,-11) (925,99) (925,51) (930,-15) (930,3) (935,51) (935,65) (940,8) (940,-4) (945,44) (945,79) (950,13) (950,-15) (955,42) (955,76) (960,-8) (960,1) (965,63) (965,82) (970,27) (970,19) (975,100) (975,57) (980,-2) (980,8) (985,63) (985,51) (990,-15) (990,-46) (995,11) (995,56) (1000,-3)}
\def\reveRawF{(0,-33) (5,10) (5,26) (10,-31) (10,-22) (15,53) (15,53) (20,-55) (20,-73) (25,16) (25,27) (30,-27) (30,-39) (35,19) (35,19) (40,-27) (40,-33) (45,30) (45,13) (50,-35) (50,-33) (55,31) (55,22) (60,-22) (60,-23) (65,22) (65,27) (70,-40) (70,-56) (75,6) (75,-17) (80,-73) (80,-80) (85,-35) (85,-10) (90,-80) (90,-63) (95,-26) (95,10) (100,-68) (100,-52) (105,20) (105,74) (110,6) (110,-42) (115,23) (115,42) (120,-36) (120,-3) (125,48) (125,53) (130,-15) (130,9) (135,58) (135,43) (140,-2) (140,-28) (145,35) (145,39) (150,-26) (150,-15) (155,36) (155,42) (160,-12) (160,-22) (165,29) (165,30) (170,-23) (170,-37) (175,23) (175,20) (180,-47) (180,-26) (185,36) (185,45) (190,-7) (190,-15) (195,37) (195,47) (200,5) (200,0) (205,81) (205,48) (210,0) (210,-7) (215,70) (215,57) (220,-24) (220,-26) (225,71) (225,70) (230,23) (230,23) (235,69) (235,76) (240,-5) (240,13) (245,66) (245,55) (250,0) (250,-35) (255,23) (255,36) (260,-20) (260,-23) (265,26) (265,35) (270,-18) (270,-21) (275,37) (275,48) (280,-20) (280,-28) (285,47) (285,75) (290,-11) (290,9) (295,71) (295,69) (300,21) (300,4) (305,78) (305,78) (310,17) (310,0) (315,71) (315,71) (320,19) (320,12) (325,73) (325,81) (330,-45) (330,-7) (335,70) (335,69) (340,20) (340,-4) (345,53) (345,62) (350,10) (350,2) (355,59) (355,41) (360,-18) (360,-21) (365,22) (365,-3) (370,-62) (370,-79) (375,-20) (375,-31) (380,-98) (380,-69) (385,-15) (385,-6) (390,-57) (390,-55) (395,24) (395,22) (400,-85) (400,-58) (405,45) (405,51) (410,-51) (410,-29) (415,64) (415,76) (420,-29) (420,-25) (425,68) (425,53) (430,-5) (430,-24) (435,34) (435,71) (440,5) (440,0) (445,74) (445,79) (450,2) (450,1) (455,93) (455,37) (460,-25) (460,-16) (465,81) (465,31) (470,-72) (470,-67) (475,21) (475,17) (480,-89) (480,-81) (485,60) (485,39) (490,-56) (490,-51) (495,71) (495,63) (500,-21) (500,-23) (505,106) (505,83) (510,15) (510,11) (515,73) (515,60) (520,-1) (520,-23) (525,68) (525,50) (530,-29) (530,-31) (535,71) (535,71) (540,-76) (540,-38) (545,31) (545,16) (550,-116) (550,-16) (555,49) (555,18) (560,-64) (560,-8) (565,54) (565,18) (570,-30) (570,-28) (575,40) (575,35) (580,-22) (580,-30) (585,34) (585,22) (590,-41) (590,-35) (595,29) (595,11) (600,-62) (600,-9) (605,39) (605,36) (610,-65) (610,3) (615,71) (615,58) (620,-30) (620,-7) (625,77) (625,68) (630,-68) (630,-38) (635,75) (635,43) (640,-57) (640,-35) (645,79) (645,27) (650,-103) (650,-41) (655,73) (655,0) (660,-82) (660,-13) (665,64) (665,-8) (670,-97) (670,-33) (675,26) (675,-10) (680,-78) (680,-45) (685,32) (685,-10) (690,-90) (690,-61) (695,11) (695,34) (700,-38) (700,-36) (705,22) (705,32) (710,-39) (710,-73) (715,33) (715,53) (720,-55) (720,-66) (725,6) (725,30) (730,-28) (730,-75) (735,9) (735,6) (740,-68) (740,-82) (745,3) (745,56) (750,-28) (750,-48) (755,10) (755,53) (760,-22) (760,-13) (765,49) (765,29) (770,-31) (770,-37) (775,28) (775,41) (780,-28) (780,-9) (785,52) (785,15) (790,-46) (790,-17) (795,39) (795,8) (800,-71) (800,-43) (805,48) (805,10) (810,-65) (810,-32) (815,68) (815,22) (820,-71) (820,-57) (825,27) (825,32) (830,-50) (830,-48) (835,36) (835,26) (840,-38) (840,-38) (845,22) (845,13) (850,-75) (850,-68) (855,27) (855,13) (860,-85) (860,-82) (865,8) (865,12) (870,-59) (870,-92) (875,5) (875,3) (880,-52) (880,-83) (885,-23) (885,30) (890,-51) (890,-69) (895,32) (895,30) (900,-28) (900,-25) (905,29) (905,27) (910,-55) (910,-39) (915,42) (915,10) (920,-81) (920,-58) (925,43) (925,-15) (930,-77) (930,-53) (935,28) (935,-4) (940,-96) (940,-65) (945,-5) (945,7) (950,-78) (950,-67) (955,16) (955,16) (960,-61) (960,-80) (965,23) (965,19) (970,-33) (970,-38) (975,15) (975,-5) (980,-61) (980,-62) (985,10) (985,12) (990,-87) (990,-116) (995,-31) (995,-7) (1000,-64)}
\def\reveRawG{(0,-51) (5,7) (5,7) (10,-56) (10,-52) (15,61) (15,19) (20,-92) (20,-98) (25,-5) (25,-2) (30,-43) (30,-56) (35,-17) (35,-12) (40,-46) (40,-51) (45,6) (45,-12) (50,-51) (50,-67) (55,-17) (55,1) (60,-35) (60,-62) (65,-11) (65,-17) (70,-76) (70,-76) (75,-39) (75,-45) (80,-116) (80,-95) (85,-56) (85,-52) (90,-111) (90,-107) (95,-43) (95,-35) (100,-124) (100,-84) (105,-24) (105,59) (110,-24) (110,-67) (115,11) (115,39) (120,-48) (120,-15) (125,44) (125,47) (130,-18) (130,-2) (135,47) (135,26) (140,-20) (140,-20) (145,35) (145,36) (150,-30) (150,-29) (155,16) (155,43) (160,-13) (160,-31) (165,23) (165,12) (170,-36) (170,-43) (175,12) (175,3) (180,-46) (180,-30) (185,32) (185,39) (190,-10) (190,-28) (195,31) (195,45) (200,5) (200,-3) (205,57) (205,34) (210,-16) (210,-22) (215,81) (215,52) (220,-42) (220,-28) (225,54) (225,58) (230,13) (230,5) (235,51) (235,51) (240,-6) (240,-8) (245,36) (245,56) (250,-26) (250,-41) (255,-2) (255,13) (260,-43) (260,-28) (265,18) (265,21) (270,-33) (270,-26) (275,19) (275,34) (280,-32) (280,-39) (285,19) (285,42) (290,-4) (290,-17) (295,43) (295,61) (300,20) (300,-4) (305,83) (305,86) (310,11) (310,-18) (315,60) (315,86) (320,28) (320,35) (325,95) (325,74) (330,-41) (330,-15) (335,56) (335,65) (340,20) (340,-10) (345,47) (345,51) (350,5) (350,3) (355,55) (355,34) (360,-19) (360,-55) (365,31) (365,1) (370,-90) (370,-115) (375,-56) (375,-54) (380,-124) (380,-108) (385,-28) (385,-15) (390,-100) (390,-43) (395,2) (395,-5) (400,-77) (400,-49) (405,29) (405,34) (410,-29) (410,-31) (415,29) (415,59) (420,-11) (420,-32) (425,37) (425,39) (430,-35) (430,-24) (435,26) (435,49) (440,-21) (440,-4) (445,74) (445,56) (450,-22) (450,8) (455,118) (455,40) (460,-47) (460,-35) (465,82) (465,-8) (470,-88) (470,-35) (475,44) (475,-8) (480,-81) (480,-55) (485,46) (485,30) (490,-40) (490,-28) (495,51) (495,56) (500,-9) (500,-3) (505,104) (505,100) (510,-20) (510,-18) (515,109) (515,110) (520,-29) (520,-28) (525,89) (525,88) (530,-60) (530,-20) (535,75) (535,73) (540,-93) (540,-24) (545,40) (545,11) (550,-101) (550,-31) (555,61) (555,52) (560,-55) (560,-17) (565,68) (565,42) (570,-24) (570,-33) (575,87) (575,74) (580,-21) (580,-15) (585,71) (585,75) (590,-53) (590,-59) (595,38) (595,34) (600,-24) (600,-14) (605,41) (605,54) (610,-44) (610,15) (615,68) (615,75) (620,-31) (620,1) (625,88) (625,97) (630,-58) (630,-23) (635,100) (635,65) (640,-54) (640,-2) (645,101) (645,44) (650,-66) (650,1) (655,90) (655,23) (660,-53) (660,-12) (665,97) (665,26) (670,-67) (670,-22) (675,60) (675,6) (680,-54) (680,-16) (685,68) (685,-4) (690,-67) (690,-33) (695,39) (695,64) (700,4) (700,8) (705,61) (705,79) (710,-4) (710,-22) (715,64) (715,68) (720,-42) (720,-32) (725,24) (725,47) (730,-2) (730,-23) (735,41) (735,35) (740,-29) (740,-34) (745,33) (745,89) (750,-10) (750,-30) (755,61) (755,72) (760,13) (760,19) (765,78) (765,64) (770,-3) (770,-16) (775,43) (775,46) (780,-23) (780,0) (785,64) (785,27) (790,-27) (790,-10) (795,43) (795,23) (800,-66) (800,-17) (805,55) (805,-9) (810,-67) (810,-13) (815,72) (815,2) (820,-64) (820,-42) (825,44) (825,1) (830,-51) (830,-24) (835,53) (835,29) (840,-27) (840,-15) (845,28) (845,15) (850,-57) (850,-43) (855,17) (855,12) (860,-44) (860,-62) (865,1) (865,13) (870,-43) (870,-74) (875,6) (875,16) (880,-25) (880,-88) (885,-9) (885,50) (890,-48) (890,-95) (895,26) (895,50) (900,-38) (900,-61) (905,14) (905,43) (910,-40) (910,-65) (915,1) (915,14) (920,-77) (920,-69) (925,31) (925,2) (930,-66) (930,-39) (935,43) (935,0) (940,-36) (940,-38) (945,21) (945,28) (950,-31) (950,-62) (955,18) (955,-5) (960,-54) (960,-53) (965,24) (965,19) (970,-28) (970,-44) (975,31) (975,15) (980,-76) (980,-62) (985,30) (985,10) (990,-99) (990,-103) (995,-37) (995,-11) (1000,-68)}
\def\reveRawH{(0,0) (5,0) (5,0) (10,0) (10,0) (15,0) (15,0) (20,0) (20,0) (25,0) (25,0) (30,0) (30,0) (35,0) (35,0) (40,0) (40,0) (45,0) (45,0) (50,0) (50,0) (55,0) (55,0) (60,0) (60,0) (65,0) (65,0) (70,0) (70,0) (75,0) (75,0) (80,0) (80,0) (85,0) (85,0) (90,0) (90,0) (95,0) (95,0) (100,0) (100,0) (105,0) (105,0) (110,0) (110,0) (115,0) (115,0) (120,0) (120,0) (125,0) (125,0) (130,0) (130,0) (135,0) (135,0) (140,0) (140,0) (145,0) (145,0) (150,0) (150,0) (155,0) (155,0) (160,0) (160,0) (165,0) (165,0) (170,0) (170,0) (175,0) (175,0) (180,0) (180,0) (185,0) (185,0) (190,0) (190,0) (195,0) (195,0) (200,0) (200,0) (205,0) (205,0) (210,0) (210,0) (215,0) (215,0) (220,0) (220,0) (225,0) (225,0) (230,0) (230,0) (235,0) (235,0) (240,0) (240,0) (245,0) (245,0) (250,0) (250,0) (255,0) (255,0) (260,0) (260,0) (265,0) (265,0) (270,0) (270,0) (275,0) (275,0) (280,0) (280,0) (285,0) (285,0) (290,0) (290,0) (295,0) (295,0) (300,0) (300,0) (305,0) (305,0) (310,0) (310,0) (315,0) (315,0) (320,0) (320,0) (325,0) (325,0) (330,0) (330,0) (335,0) (335,0) (340,0) (340,0) (345,0) (345,0) (350,0) (350,0) (355,80) (355,80) (360,0) (360,0) (365,0) (365,0) (370,0) (370,0) (375,0) (375,0) (380,0) (380,0) (385,0) (385,0) (390,0) (390,0) (395,0) (395,0) (400,0) (400,0) (405,0) (405,0) (410,0) (410,0) (415,0) (415,0) (420,0) (420,0) (425,0) (425,0) (430,0) (430,0) (435,0) (435,0) (440,0) (440,0) (445,0) (445,0) (450,0) (450,0) (455,0) (455,0) (460,0) (460,0) (465,0) (465,0) (470,0) (470,0) (475,0) (475,0) (480,0) (480,0) (485,0) (485,0) (490,0) (490,0) (495,0) (495,0) (500,0) (500,0) (505,0) (505,0) (510,0) (510,0) (515,0) (515,0) (520,0) (520,0) (525,0) (525,0) (530,0) (530,0) (535,0) (535,0) (540,0) (540,0) (545,0) (545,0) (550,0) (550,0) (555,0) (555,0) (560,0) (560,0) (565,0) (565,0) (570,0) (570,0) (575,0) (575,0) (580,0) (580,0) (585,0) (585,0) (590,0) (590,0) (595,0) (595,0) (600,0) (600,0) (605,0) (605,0) (610,0) (610,0) (615,0) (615,0) (620,0) (620,0) (625,0) (625,0) (630,0) (630,0) (635,0) (635,0) (640,0) (640,0) (645,0) (645,0) (650,0) (650,0) (655,0) (655,0) (660,0) (660,0) (665,0) (665,0) (670,0) (670,0) (675,0) (675,0) (680,0) (680,0) (685,0) (685,0) (690,0) (690,0) (695,0) (695,0) (700,0) (700,0) (705,0) (705,0) (710,0) (710,0) (715,0) (715,0) (720,0) (720,0) (725,0) (725,0) (730,0) (730,0) (735,0) (735,0) (740,0) (740,0) (745,0) (745,0) (750,0) (750,0) (755,0) (755,0) (760,0) (760,0) (765,0) (765,0) (770,0) (770,0) (775,0) (775,0) (780,0) (780,0) (785,0) (785,0) (790,0) (790,0) (795,0) (795,0) (800,0) (800,0) (805,0) (805,0) (810,0) (810,0) (815,0) (815,0) (820,0) (820,0) (825,0) (825,0) (830,0) (830,0) (835,0) (835,0) (840,0) (840,0) (845,0) (845,0) (850,0) (850,0) (855,0) (855,0) (860,0) (860,0) (865,0) (865,0) (870,0) (870,0) (875,0) (875,0) (880,0) (880,0) (885,0) (885,0) (890,0) (890,0) (895,0) (895,0) (900,0) (900,0) (905,0) (905,0) (910,0) (910,0) (915,0) (915,0) (920,0) (920,0) (925,0) (925,0) (930,0) (930,0) (935,0) (935,0) (940,0) (940,0) (945,0) (945,0) (950,0) (950,0) (955,0) (955,0) (960,0) (960,0) (965,0) (965,0) (970,0) (970,0) (975,0) (975,0) (980,0) (980,0) (985,0) (985,0) (990,0) (990,0) (995,0) (995,0) (1000,0)}
\def\reveTraceA{(0,-44) (4,29) (6,25) (9,-42) (10,-41) (14,24) (16,18) (19,-47) (20,-38) (24,25) (26,21) (29,-42) (30,-41) (34,24) (36,30) (39,-36) (40,-38) (44,31) (46,30) (49,-36) (50,-37) (54,27) (56,28) (59,-42) (60,-31) (64,37) (66,30) (69,-38) (70,-31) (74,56) (76,75) (79,-7) (80,15) (84,86) (86,82) (89,-3) (90,-20) (94,61) (96,45) (99,-34) (100,-44) (104,33) (106,25) (109,-55) (110,-52) (114,23) (116,23) (119,-55) (120,-50) (124,26) (126,26) (129,-52) (130,-48) (134,26) (136,28) (139,-53) (140,-54) (144,30) (146,31) (149,-45) (150,-48) (154,32) (156,29) (159,-52) (160,-53) (164,28) (166,28) (169,-51) (170,-48) (174,30) (176,31) (179,-57) (180,-56) (184,26) (186,24) (189,-55) (190,-53) (194,26) (196,23) (199,-59) (200,-42) (204,38) (206,37) (209,-46) (210,-48) (214,37) (216,33) (219,-52) (220,-52) (224,34) (226,34) (229,-50) (230,-52) (234,41) (236,35) (239,-51) (240,-47) (244,38) (246,30) (249,-53) (250,-46) (254,37) (256,31) (259,-52) (260,-56) (264,28) (266,31) (269,-58) (270,-58) (274,27) (276,32) (279,-55) (280,-57) (284,33) (286,29) (289,-56) (290,-53) (294,37) (296,25) (299,-64) (300,-62) (304,31) (306,18) (309,-70) (310,-76) (314,14) (316,13) (319,-81) (320,-81) (324,9) (326,15) (329,-81) (330,-77) (334,13) (336,9) (339,-78) (340,-75) (344,12) (346,25) (349,-76) (350,-45) (354,43) (356,53) (359,-38) (360,-25) (364,65) (366,63) (369,-27) (370,-25) (374,66) (376,70) (379,-28) (380,-12) (384,76) (386,81) (389,-14) (390,-20) (394,70) (396,57) (399,-33) (400,-30) (404,57) (406,47) (409,-42) (410,-36) (414,53) (416,48) (419,-43) (420,-40) (424,53) (426,48) (429,-46) (430,-38) (434,50) (436,49) (439,-43) (440,-51) (444,45) (446,44) (449,-54) (450,-48) (454,43) (456,47) (459,-45) (460,-45) (464,47) (466,43) (469,-47) (470,-50) (474,45) (476,48) (479,-43) (480,-51) (484,43) (486,44) (489,-52) (490,-52) (494,38) (496,41) (499,-56) (500,-56) (504,31) (506,29) (509,-61) (510,-57) (514,32) (516,33) (519,-58) (520,-48) (524,37) (526,44) (529,-47) (530,-44) (534,43) (536,41) (539,-44) (540,-40) (544,44) (546,42) (549,-47) (550,-42) (554,46) (556,36) (559,-49) (560,-43) (564,41) (566,33) (569,-53) (570,-54) (574,36) (576,29) (579,-55) (580,-49) (584,35) (586,30) (589,-50) (590,-42) (594,43) (596,39) (599,-44) (600,-37) (604,44) (606,38) (609,-47) (610,-44) (614,45) (616,39) (619,-45) (620,-45) (624,40) (626,32) (629,-51) (630,-50) (634,32) (636,40) (639,-45) (640,-45) (644,35) (646,34) (649,-49) (650,-45) (654,34) (656,30) (659,-49) (660,-48) (664,29) (666,32) (669,-46) (670,-44) (674,39) (676,39) (679,-40) (680,-40) (684,38) (686,38) (689,-35) (690,-32) (694,42) (696,35) (699,-38) (700,-38) (704,37) (706,31) (709,-41) (710,-39) (714,36) (716,30) (719,-47) (720,-38) (724,33) (726,26) (729,-44) (730,-43) (734,31) (736,32) (739,-39) (740,-45) (744,27) (746,22) (749,-44) (750,-42) (754,26) (756,28) (759,-44) (760,-44) (764,30) (766,26) (769,-44) (770,-39) (774,29) (776,31) (779,-42) (780,-43) (784,32) (786,30) (789,-41) (790,-35) (794,30) (796,27) (799,-42) (800,-40) (804,31) (806,40) (809,-27) (810,-30) (814,37) (816,34) (819,-38) (820,-37) (824,35) (826,32) (829,-42) (830,-50) (834,29) (836,29) (839,-45) (840,-43) (844,26) (846,35) (849,-36) (850,-37) (854,36) (856,32) (859,-51) (860,-46) (864,32) (866,24) (869,-49) (870,-47) (874,30) (876,32) (879,-45) (880,-40) (884,37) (886,40) (889,-34) (890,-40) (894,40) (896,31) (899,-46) (900,-42) (904,45) (906,41) (909,-40) (910,-45) (914,45) (916,40) (919,-43) (920,-38) (924,41) (926,37) (929,-40) (930,-49) (934,33) (936,28) (939,-54) (940,-57) (944,29) (946,24) (949,-56) (950,-54) (954,32) (956,23) (959,-58) (960,-55) (964,27) (966,31) (969,-56) (970,-62) (974,25) (976,31) (979,-53) (980,-49) (984,43) (986,52) (989,-32) (990,-28) (994,56) (996,66) (999,-18)}
\def\reveTraceB{(0,-43) (4,15) (6,23) (9,-26) (10,-23) (14,24) (16,6) (19,-37) (20,-12) (24,25) (26,22) (29,-23) (30,-16) (34,23) (36,38) (39,-9) (40,-13) (44,41) (46,41) (49,-9) (50,-8) (54,36) (56,32) (59,-23) (60,-2) (64,49) (66,39) (69,-7) (70,9) (74,79) (76,100) (79,43) (80,84) (84,100) (86,100) (89,47) (90,16) (94,69) (96,52) (99,-9) (100,-26) (104,37) (106,14) (109,-48) (110,-45) (114,10) (116,0) (119,-57) (120,-38) (124,11) (126,15) (129,-42) (130,-34) (134,14) (136,14) (139,-42) (140,-51) (144,14) (146,19) (149,-30) (150,-33) (154,15) (156,9) (159,-44) (160,-49) (164,3) (166,13) (169,-38) (170,-37) (174,10) (176,0) (179,-71) (180,-64) (184,-4) (186,-12) (189,-60) (190,-57) (194,-8) (196,-14) (199,-62) (200,-29) (204,27) (206,32) (209,-25) (210,-33) (214,30) (216,17) (219,-38) (220,-36) (224,17) (226,21) (229,-40) (230,-40) (234,40) (236,27) (239,-35) (240,-23) (244,39) (246,21) (249,-31) (250,-21) (254,37) (256,22) (259,-31) (260,-36) (264,17) (266,21) (269,-38) (270,-45) (274,17) (276,20) (279,-40) (280,-48) (284,25) (286,15) (289,-39) (290,-30) (294,33) (296,-3) (299,-59) (300,-68) (304,7) (306,-23) (309,-82) (310,-88) (314,-31) (316,-32) (319,-100) (320,-100) (324,-39) (326,-33) (329,-100) (330,-95) (334,-35) (336,-49) (339,-100) (340,-100) (344,-35) (346,-21) (349,-100) (350,-38) (354,21) (356,53) (359,-13) (360,15) (364,74) (366,75) (369,16) (370,26) (374,89) (376,90) (379,17) (380,54) (384,100) (386,100) (389,59) (390,43) (394,100) (396,70) (399,7) (400,10) (404,69) (406,46) (409,-11) (410,8) (414,63) (416,48) (419,-6) (420,1) (424,68) (426,52) (429,-10) (430,3) (434,59) (436,58) (439,-8) (440,-25) (444,46) (446,49) (449,-30) (450,-26) (454,39) (456,54) (459,-11) (460,-5) (464,53) (466,49) (469,-11) (470,-26) (474,35) (476,40) (479,-18) (480,-32) (484,39) (486,43) (489,-34) (490,-34) (494,22) (496,26) (499,-54) (500,-52) (504,10) (506,4) (509,-54) (510,-46) (514,15) (516,14) (519,-52) (520,-34) (524,19) (526,29) (529,-39) (530,-31) (534,31) (536,38) (539,-26) (540,-17) (544,35) (546,30) (549,-26) (550,-7) (554,50) (556,30) (559,-20) (560,-11) (564,43) (566,9) (569,-47) (570,-50) (574,11) (576,-1) (579,-54) (580,-42) (584,13) (586,-3) (589,-50) (590,-26) (594,29) (596,15) (599,-37) (600,-15) (604,41) (606,29) (609,-35) (610,-23) (614,43) (616,38) (619,-29) (620,-17) (624,34) (626,22) (629,-40) (630,-31) (634,19) (636,26) (639,-32) (640,-24) (644,30) (646,19) (649,-38) (650,-22) (654,33) (656,16) (659,-42) (660,-39) (664,14) (666,11) (669,-35) (670,-28) (674,27) (676,25) (679,-28) (680,-21) (684,38) (686,22) (689,-21) (690,-11) (694,33) (696,32) (699,-19) (700,-26) (704,23) (706,10) (709,-39) (710,-27) (714,23) (716,27) (719,-39) (720,-12) (724,34) (726,16) (729,-29) (730,-34) (734,20) (736,38) (739,-11) (740,-24) (744,26) (746,21) (749,-20) (750,-23) (754,23) (756,33) (759,-22) (760,-23) (764,38) (766,29) (769,-20) (770,-20) (774,31) (776,46) (779,-22) (780,-25) (784,44) (786,37) (789,-22) (790,-6) (794,47) (796,30) (799,-26) (800,-18) (804,35) (806,46) (809,-4) (810,3) (814,44) (816,36) (819,-25) (820,-15) (824,42) (826,32) (829,-20) (830,-39) (834,26) (836,27) (839,-38) (840,-21) (844,23) (846,31) (849,-12) (850,-14) (854,39) (856,26) (859,-38) (860,-32) (864,26) (866,11) (869,-36) (870,-37) (874,16) (876,17) (879,-34) (880,-27) (884,25) (886,34) (889,-14) (890,-26) (894,33) (896,18) (899,-38) (900,-22) (904,43) (906,37) (909,-17) (910,-29) (914,56) (916,39) (919,-29) (920,-6) (924,47) (926,33) (929,-12) (930,-35) (934,18) (936,13) (939,-35) (940,-53) (944,7) (946,4) (949,-46) (950,-42) (954,26) (956,19) (959,-46) (960,-39) (964,16) (966,30) (969,-36) (970,-49) (974,14) (976,32) (979,-36) (980,-17) (984,56) (986,63) (989,10) (990,9) (994,71) (996,92) (999,37)}
\def\reveTraceC{(0,-38) (4,34) (6,35) (9,-36) (10,-40) (14,32) (16,27) (19,-40) (20,-37) (24,39) (26,23) (29,-46) (30,-36) (34,28) (36,35) (39,-35) (40,-31) (44,40) (46,43) (49,-33) (50,-35) (54,35) (56,27) (59,-43) (60,-29) (64,42) (66,33) (69,-34) (70,-29) (74,53) (76,62) (79,-11) (80,-4) (84,68) (86,68) (89,-18) (90,-25) (94,48) (96,48) (99,-38) (100,-50) (104,34) (106,20) (109,-59) (110,-58) (114,22) (116,25) (119,-54) (120,-53) (124,28) (126,30) (129,-48) (130,-51) (134,28) (136,35) (139,-48) (140,-53) (144,40) (146,40) (149,-38) (150,-44) (154,38) (156,35) (159,-47) (160,-49) (164,33) (166,37) (169,-46) (170,-40) (174,37) (176,45) (179,-46) (180,-48) (184,37) (186,28) (189,-52) (190,-42) (194,39) (196,30) (199,-52) (200,-41) (204,40) (206,46) (209,-41) (210,-48) (214,45) (216,40) (219,-45) (220,-58) (224,40) (226,34) (229,-53) (230,-52) (234,52) (236,40) (239,-48) (240,-37) (244,45) (246,27) (249,-54) (250,-37) (254,46) (256,31) (259,-54) (260,-54) (264,29) (266,30) (269,-59) (270,-55) (274,33) (276,44) (279,-46) (280,-49) (284,48) (286,39) (289,-49) (290,-34) (294,56) (296,32) (299,-56) (300,-46) (304,47) (306,37) (309,-63) (310,-60) (314,33) (316,28) (319,-68) (320,-71) (324,23) (326,32) (329,-65) (330,-59) (334,35) (336,23) (339,-65) (340,-57) (344,30) (346,37) (349,-63) (350,-53) (354,34) (356,50) (359,-50) (360,-43) (364,56) (366,56) (369,-36) (370,-28) (374,67) (376,71) (379,-27) (380,-13) (384,78) (386,78) (389,-22) (390,-28) (394,59) (396,56) (399,-37) (400,-37) (404,56) (406,41) (409,-51) (410,-47) (414,49) (416,43) (419,-54) (420,-41) (424,57) (426,50) (429,-49) (430,-39) (434,57) (436,57) (439,-45) (440,-51) (444,48) (446,53) (449,-52) (450,-55) (454,41) (456,51) (459,-44) (460,-42) (464,51) (466,52) (469,-41) (470,-44) (474,55) (476,63) (479,-38) (480,-54) (484,44) (486,54) (489,-45) (490,-47) (494,45) (496,54) (499,-47) (500,-52) (504,34) (506,27) (509,-62) (510,-56) (514,36) (516,38) (519,-58) (520,-47) (524,42) (526,54) (529,-43) (530,-39) (534,54) (536,45) (539,-47) (540,-35) (544,53) (546,53) (549,-41) (550,-42) (554,51) (556,37) (559,-52) (560,-39) (564,47) (566,37) (569,-55) (570,-53) (574,44) (576,38) (579,-57) (580,-45) (584,41) (586,36) (589,-49) (590,-35) (594,52) (596,47) (599,-37) (600,-31) (604,57) (606,41) (609,-46) (610,-47) (614,50) (616,43) (619,-47) (620,-47) (624,44) (626,40) (629,-55) (630,-49) (634,34) (636,44) (639,-46) (640,-46) (644,38) (646,43) (649,-49) (650,-49) (654,36) (656,36) (659,-50) (660,-46) (664,35) (666,40) (669,-44) (670,-47) (674,32) (676,35) (679,-48) (680,-44) (684,40) (686,49) (689,-29) (690,-26) (694,54) (696,36) (699,-38) (700,-39) (704,45) (706,34) (709,-43) (710,-38) (714,42) (716,29) (719,-50) (720,-42) (724,37) (726,33) (729,-48) (730,-39) (734,40) (736,40) (739,-37) (740,-43) (744,31) (746,31) (749,-47) (750,-44) (754,26) (756,23) (759,-50) (760,-49) (764,27) (766,34) (769,-47) (770,-41) (774,38) (776,36) (779,-43) (780,-46) (784,33) (786,41) (789,-37) (790,-38) (794,36) (796,40) (799,-37) (800,-34) (804,42) (806,53) (809,-19) (810,-29) (814,43) (816,40) (819,-34) (820,-33) (824,42) (826,44) (829,-37) (830,-52) (834,44) (836,41) (839,-45) (840,-39) (844,29) (846,53) (849,-25) (850,-25) (854,45) (856,48) (859,-49) (860,-43) (864,45) (866,36) (869,-41) (870,-43) (874,43) (876,44) (879,-42) (880,-33) (884,47) (886,43) (889,-32) (890,-39) (894,48) (896,29) (899,-48) (900,-45) (904,44) (906,40) (909,-50) (910,-54) (914,45) (916,40) (919,-50) (920,-52) (924,32) (926,30) (929,-50) (930,-62) (934,25) (936,24) (939,-69) (940,-70) (944,18) (946,15) (949,-66) (950,-62) (954,32) (956,23) (959,-58) (960,-57) (964,37) (966,36) (969,-57) (970,-66) (974,29) (976,41) (979,-45) (980,-49) (984,41) (986,60) (989,-31) (990,-27) (994,57) (996,65) (999,-24)}
\def\reveTraceD{(0,-64) (4,-6) (6,35) (9,-32) (10,-40) (14,31) (16,12) (19,-68) (20,-40) (24,41) (26,25) (29,-18) (30,8) (34,44) (36,49) (39,2) (40,4) (44,53) (46,62) (49,-11) (50,9) (54,55) (56,55) (59,4) (60,14) (64,63) (66,35) (69,1) (70,5) (74,40) (76,75) (79,-18) (80,14) (84,59) (86,51) (89,18) (90,-26) (94,36) (96,53) (99,-24) (100,-28) (104,35) (106,32) (109,-48) (110,-36) (114,14) (116,-1) (119,-76) (120,-10) (124,35) (126,15) (129,-37) (130,-17) (134,26) (136,16) (139,-28) (140,-46) (144,5) (146,8) (149,-23) (150,-22) (154,9) (156,-5) (159,-45) (160,-59) (164,-15) (166,0) (169,-37) (170,-54) (174,-14) (176,-21) (179,-94) (180,-68) (184,-22) (186,-19) (189,-60) (190,-57) (194,-14) (196,-19) (199,-72) (200,-21) (204,17) (206,47) (209,-42) (210,-32) (214,30) (216,14) (219,-47) (220,-50) (224,43) (226,52) (229,-48) (230,-7) (234,79) (236,31) (239,-25) (240,-21) (244,56) (246,24) (249,-43) (250,-54) (254,23) (256,41) (259,-33) (260,-35) (264,16) (266,28) (269,-38) (270,-47) (274,7) (276,12) (279,-51) (280,-21) (284,59) (286,49) (289,-21) (290,-14) (294,74) (296,16) (299,-43) (300,-71) (304,33) (306,-8) (309,-52) (310,-78) (314,5) (316,7) (319,-100) (320,-86) (324,-1) (326,-34) (329,-100) (330,-52) (334,-5) (336,-32) (339,-86) (340,-81) (344,-12) (346,6) (349,-87) (350,-41) (354,8) (356,33) (359,-27) (360,-15) (364,39) (366,6) (369,-25) (370,-20) (374,33) (376,36) (379,-43) (380,28) (384,69) (386,85) (389,38) (390,12) (394,90) (396,46) (399,-21) (400,-19) (404,61) (406,24) (409,-38) (410,1) (414,45) (416,55) (419,-27) (420,6) (424,83) (426,59) (429,-31) (430,-23) (434,91) (436,77) (439,-23) (440,-33) (444,49) (446,75) (449,0) (450,-28) (454,73) (456,97) (459,-43) (460,25) (464,75) (466,8) (469,-52) (470,-25) (474,20) (476,11) (479,-47) (480,-34) (484,31) (486,40) (489,-45) (490,-49) (494,26) (496,13) (499,-69) (500,-56) (504,49) (506,11) (509,-39) (510,-21) (514,45) (516,48) (519,-61) (520,-39) (524,29) (526,34) (529,-25) (530,-64) (534,57) (536,66) (539,-48) (540,-10) (544,40) (546,5) (549,-47) (550,12) (554,54) (556,26) (559,-20) (560,-10) (564,46) (566,-18) (569,-66) (570,-63) (574,-8) (576,-17) (579,-73) (580,-60) (584,12) (586,-13) (589,-74) (590,-14) (594,52) (596,23) (599,-86) (600,-25) (604,51) (606,46) (609,-45) (610,1) (614,61) (616,43) (619,-2) (620,-5) (624,46) (626,28) (629,-49) (630,-35) (634,50) (636,22) (639,-70) (640,-47) (644,57) (646,21) (649,-89) (650,-41) (654,48) (656,-10) (659,-52) (660,-36) (664,5) (666,5) (669,-49) (670,-21) (674,36) (676,-3) (679,-45) (680,-40) (684,39) (686,-7) (689,-47) (690,-22) (694,19) (696,22) (699,-27) (700,-52) (704,10) (706,0) (709,-58) (710,-57) (714,35) (716,13) (719,-28) (720,-23) (724,16) (726,26) (729,-43) (730,-54) (734,-9) (736,39) (739,-21) (740,-83) (744,14) (746,45) (749,-19) (750,-39) (754,30) (756,34) (759,-9) (760,-8) (764,70) (766,43) (769,-14) (770,-34) (774,48) (776,77) (779,-22) (780,-4) (784,71) (786,66) (789,10) (790,-6) (794,66) (796,2) (799,-59) (800,-9) (804,45) (806,58) (809,-53) (810,-6) (814,81) (816,44) (819,-29) (820,-34) (824,57) (826,72) (829,6) (830,-19) (834,24) (836,50) (839,-23) (840,-14) (844,61) (846,43) (849,-34) (850,-2) (854,75) (856,9) (859,-35) (860,-38) (864,13) (866,15) (869,-26) (870,-48) (874,6) (876,15) (879,-39) (880,-37) (884,18) (886,39) (889,-20) (890,-23) (894,48) (896,28) (899,-23) (900,1) (904,51) (906,38) (909,-4) (910,-30) (914,92) (916,18) (919,-45) (920,-28) (924,63) (926,34) (929,-39) (930,-34) (934,36) (936,28) (939,-17) (940,-66) (944,-23) (946,27) (949,-41) (950,-65) (954,29) (956,61) (959,-69) (960,-38) (964,28) (966,25) (969,-30) (970,-20) (974,30) (976,37) (979,-44) (980,3) (984,58) (986,39) (989,-2) (990,-31) (994,37) (996,65) (999,6)}
\def\reveTraceE{(0,-17) (4,36) (6,50) (9,-12) (10,7) (14,87) (16,45) (19,-49) (20,-39) (24,51) (26,40) (29,-4) (30,-10) (34,43) (36,42) (39,-16) (40,-12) (44,23) (46,29) (49,-21) (50,-24) (54,19) (56,21) (59,-18) (60,-19) (64,21) (66,11) (69,-30) (70,-51) (74,-10) (76,-32) (79,-66) (80,-89) (84,-43) (86,-49) (89,-81) (90,-66) (94,-21) (96,-20) (99,-73) (100,-35) (104,26) (106,59) (109,7) (110,-12) (114,37) (116,45) (119,-27) (120,10) (124,51) (126,43) (129,-22) (130,14) (134,48) (136,34) (139,-12) (140,-13) (144,50) (146,8) (149,-20) (150,-23) (154,19) (156,26) (159,-23) (160,-31) (164,27) (166,20) (169,-22) (170,-34) (174,5) (176,-11) (179,-55) (180,-41) (184,11) (186,12) (189,-54) (190,-59) (194,-18) (196,6) (199,-47) (200,-14) (204,24) (206,14) (209,-34) (210,-8) (214,42) (216,27) (219,-66) (220,-44) (224,44) (226,38) (229,-1) (230,21) (234,47) (236,9) (239,-46) (240,-17) (244,28) (246,35) (249,-37) (250,-67) (254,-26) (256,-9) (259,-51) (260,-65) (264,-14) (266,-6) (269,-54) (270,-71) (274,-12) (276,-13) (279,-57) (280,-40) (284,20) (286,43) (289,-17) (290,-5) (294,60) (296,34) (299,-9) (300,-27) (304,24) (306,37) (309,0) (310,-24) (314,53) (316,55) (319,1) (320,3) (324,48) (326,8) (329,-67) (330,-8) (334,38) (336,47) (339,-1) (340,-6) (344,51) (346,63) (349,5) (350,10) (354,56) (356,63) (359,9) (360,-18) (364,46) (366,-1) (369,-43) (370,-64) (374,-11) (376,-40) (379,-88) (380,-56) (384,-2) (386,-1) (389,-57) (390,-58) (394,23) (396,-15) (399,-71) (400,-25) (404,23) (406,17) (409,-68) (410,-30) (414,52) (416,63) (419,-41) (420,-26) (424,70) (426,48) (429,-29) (430,-8) (434,62) (436,90) (439,27) (440,15) (444,89) (446,84) (449,14) (450,78) (454,100) (456,67) (459,-9) (460,22) (464,69) (466,0) (469,-67) (470,-21) (474,9) (476,-1) (479,-49) (480,-25) (484,66) (486,20) (489,-36) (490,-39) (494,55) (496,43) (499,-23) (500,-20) (504,96) (506,51) (509,10) (510,17) (514,54) (516,50) (519,-5) (520,-20) (524,41) (526,20) (529,-41) (530,-81) (534,31) (536,28) (539,-85) (540,-41) (544,46) (546,2) (549,-68) (550,1) (554,68) (556,30) (559,-19) (560,-14) (564,52) (566,35) (569,-17) (570,-18) (574,26) (576,3) (579,-53) (580,-56) (584,-8) (586,5) (589,-65) (590,-52) (594,11) (596,7) (599,-60) (600,-24) (604,16) (606,19) (609,-58) (610,-17) (614,32) (616,14) (619,-41) (620,-34) (624,31) (626,31) (629,-53) (630,-39) (634,58) (636,17) (639,-73) (640,-33) (644,52) (646,16) (649,-100) (650,-49) (654,54) (656,-1) (659,-82) (660,-36) (664,34) (666,-25) (669,-81) (670,-33) (674,6) (676,-33) (679,-76) (680,-48) (684,5) (686,-28) (689,-85) (690,-52) (694,27) (696,28) (699,-14) (700,-31) (704,39) (706,59) (709,-17) (710,-53) (714,43) (716,79) (719,-13) (720,-58) (724,17) (726,60) (729,-6) (730,-71) (734,7) (736,25) (739,-57) (740,-100) (744,21) (746,76) (749,-27) (750,-54) (754,47) (756,55) (759,-8) (760,5) (764,55) (766,30) (769,-27) (770,-10) (774,40) (776,59) (779,2) (780,-22) (784,49) (786,32) (789,-30) (790,-4) (794,36) (796,5) (799,-52) (800,3) (804,52) (806,17) (809,-48) (810,26) (814,74) (816,26) (819,-19) (820,1) (824,54) (826,53) (829,11) (830,10) (834,73) (836,51) (839,9) (840,2) (844,59) (846,42) (849,-20) (850,-28) (854,50) (856,19) (859,-44) (860,-53) (864,-6) (866,-5) (869,-25) (870,-51) (874,7) (876,14) (879,-22) (880,-68) (884,11) (886,36) (889,-54) (890,-47) (894,38) (896,40) (899,-13) (900,-3) (904,41) (906,47) (909,-24) (910,-16) (914,52) (916,2) (919,-28) (920,-26) (924,57) (926,8) (929,-45) (930,-31) (934,5) (936,23) (939,-29) (940,-33) (944,5) (946,33) (949,-23) (950,-46) (954,2) (956,32) (959,-39) (960,-35) (964,17) (966,31) (969,-5) (970,-14) (974,47) (976,3) (979,-38) (980,-22) (984,14) (986,7) (989,-54) (990,-87) (994,-35) (996,2) (999,-37)}
\def\reveTraceF{(0,-15) (4,24) (6,23) (9,-15) (10,-20) (14,86) (16,44) (19,-57) (20,-59) (24,15) (26,23) (29,-10) (30,-9) (34,3) (36,9) (39,-11) (40,-23) (44,25) (46,7) (49,-21) (50,-26) (54,9) (56,21) (59,-9) (60,-32) (64,10) (66,3) (69,-34) (70,-50) (74,-23) (76,-28) (79,-76) (80,-68) (84,-40) (86,-45) (89,-80) (90,-74) (94,-30) (96,-18) (99,-94) (100,-62) (104,-16) (106,72) (109,-3) (110,-47) (114,18) (116,49) (119,-33) (120,6) (124,57) (126,58) (129,-2) (130,14) (134,54) (136,30) (139,-8) (140,-8) (144,40) (146,36) (149,-18) (150,-22) (154,17) (156,38) (159,2) (160,-21) (164,20) (166,10) (169,-23) (170,-37) (174,10) (176,-3) (179,-39) (180,-24) (184,25) (186,32) (189,-1) (190,-27) (194,18) (196,36) (199,9) (200,-4) (204,48) (206,17) (209,-14) (210,-15) (214,65) (216,46) (219,-42) (220,-27) (224,45) (226,47) (229,13) (230,2) (234,39) (236,35) (239,-5) (240,-7) (244,19) (246,41) (249,-15) (250,-47) (254,-17) (256,-3) (259,-40) (260,-35) (264,-8) (266,2) (269,-33) (270,-35) (274,7) (276,14) (279,-32) (280,-40) (284,-1) (286,22) (289,-11) (290,-21) (294,18) (296,45) (299,18) (300,0) (304,36) (306,75) (309,17) (310,-16) (314,37) (316,64) (319,29) (320,36) (324,77) (326,61) (329,-38) (330,-20) (334,38) (336,55) (339,15) (340,-11) (344,39) (346,46) (349,3) (350,-1) (354,42) (356,29) (359,-18) (360,-59) (364,22) (366,-7) (369,-62) (370,-100) (374,-62) (376,-60) (379,-100) (380,-100) (384,-37) (386,-27) (389,-92) (390,-38) (394,-9) (396,-12) (399,-72) (400,-42) (404,5) (406,26) (409,-28) (410,-30) (414,23) (416,54) (419,-14) (420,-30) (424,23) (426,35) (429,-11) (430,-30) (434,18) (436,30) (439,-19) (440,1) (444,68) (446,51) (449,-25) (450,2) (454,100) (456,32) (459,-48) (460,-32) (464,73) (466,-17) (469,-87) (470,-41) (474,36) (476,-17) (479,-80) (480,-58) (484,30) (486,24) (489,-40) (490,-35) (494,27) (496,45) (499,-12) (500,-11) (504,87) (506,86) (509,-18) (510,-26) (514,91) (516,92) (519,-36) (520,-32) (524,65) (526,73) (529,-68) (530,-28) (534,40) (536,58) (539,-100) (540,-36) (544,23) (546,1) (549,-100) (550,-36) (554,46) (556,38) (559,-62) (560,-34) (564,45) (566,32) (569,-20) (570,-40) (574,49) (576,63) (579,-25) (580,-23) (584,36) (586,57) (589,-54) (590,-69) (594,6) (596,11) (599,-35) (600,-28) (604,18) (606,32) (609,-59) (610,5) (614,48) (616,51) (619,-45) (620,-9) (624,56) (626,77) (629,-69) (630,-35) (634,79) (636,45) (639,-61) (640,4) (644,75) (646,22) (649,-77) (650,-8) (654,64) (656,0) (659,-64) (660,-16) (664,80) (666,4) (669,-77) (670,-29) (674,37) (676,-14) (679,-68) (680,-26) (684,47) (686,-18) (689,-71) (690,-46) (694,13) (696,35) (699,-3) (700,-2) (704,39) (706,58) (709,1) (710,-33) (714,36) (716,47) (719,-37) (720,-43) (724,-4) (726,30) (729,-5) (730,-26) (734,20) (736,26) (739,-35) (740,-38) (744,17) (746,73) (749,-12) (750,-38) (754,45) (756,55) (759,6) (760,12) (764,66) (766,49) (769,1) (770,-13) (774,27) (776,33) (779,-14) (780,-10) (784,53) (786,14) (789,-31) (790,-6) (794,38) (796,22) (799,-61) (800,-16) (804,38) (806,-13) (809,-65) (810,-19) (814,66) (816,5) (819,-57) (820,-47) (824,38) (826,6) (829,-39) (830,-28) (834,54) (836,33) (839,-10) (840,-8) (844,23) (846,22) (849,-45) (850,-37) (854,18) (856,21) (859,-30) (860,-44) (864,5) (866,20) (869,-29) (870,-55) (874,7) (876,22) (879,-9) (880,-67) (884,-4) (886,53) (889,-29) (890,-70) (894,35) (896,60) (899,-15) (900,-35) (904,23) (906,54) (909,-10) (910,-41) (914,12) (916,19) (919,-53) (920,-51) (924,34) (926,13) (929,-44) (930,-16) (934,47) (936,14) (939,-15) (940,-17) (944,36) (946,34) (949,-5) (950,-33) (954,29) (956,12) (959,-28) (960,-34) (964,31) (966,28) (969,-8) (970,-22) (974,34) (976,30) (979,-53) (980,-38) (984,28) (986,24) (989,-80) (990,-82) (994,-36) (996,-1) (999,-53)}

